M2K: Making the Model-Kernel Interface Explicit for Reliable CUDA Kernel Verification

Large language model (LLM) inference systems rely on CUDA kernels for core GPU computations, yet the interface between models and kernels is implicit and poorly specified. Models and kernels evolve independently and often make incompatible assumptions about tensor shapes and input sizes, leading to subtle memory bugs in CUDA kernels. These bugs can crash inference services, corrupt model weights, or be exploited by remote adversaries. Existing techniques either incur prohibitive runtime overhead, require specialized hardware, or fail to handle dynamic tensor shapes and variable kernel launch configurations, leaving the CUDA memory bugs largely unaddressed. This paper presents M2K, a fully automated framework that makes the model-kernel interface explicit and leverages it to detect memory bugs in CUDA kernels used in LLM inference systems. M2K consists of two components. HFProbe traces model execution without GPU hardware, classifies kernel arguments into model-fixed and user-variable, and emits symbolic constraints that capture the interface. cuKLEE then performs symbolic execution on CUDA kernels to pinpoint memory bugs under the interface constraints, modeling tensors as disjoint memory regions and treating thread identifiers symbolically to scale to thousands of threads. In the evaluation, M2K discovers 181 previously unknown bugs in real LLM inference systems, while producing only nine false positives, demonstrating its effectiveness.

==> figure/fig-running-example.tex <==
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.97\columnwidth}
\begin{tcolorbox}[colback=white!95!gray,% background color
boxrule=0.3pt, % thin border
left=0.5mm, right=0.5mm, top=0mm, bottom=0.2mm,
fontupper=\ttfamily\footnotesize,
valign=top, 
]
\begin{tabular}{@{}r@{\quad }l} % r = line numbers, l = math content
1 & $\displaystyle 1 \leq BS \leq 1000,\ 1 \leq SL \leq 1{,}000{,}000,\ TC \leq 10{,}000{,}000,$ \\[2pt]
2 & $\displaystyle D_{i} = 2,\ d^0_{i} = TC,\ d^1_{i} = 7168,\ N_{i} = TC \times 7168,\ S_{\text{i}} = 2,$ \\[2pt]
3 & $\displaystyle D_{r} = 2,\ d^0_{r} = TC,\ d^1_{r} = 7168,\ N_{r} = N_{i},\ S_{i} = 2,...$ \\
\end{tabular}
\end{tcolorbox}
    \vspace{-0.1in}
    \subcaption{XXXX}
    \label{fig:running-a}

\begin{tcolorbox}[colback=white!95!gray,% background color
boxrule=0.3pt, % thin border
left=0.5mm, right=0.5mm, top=0mm, bottom=0.2mm,
fontupper=\ttfamily\footnotesize,
valign=top, 
]
\noindent
\begin{tabular}{@{}r@{\quad }l} % r = line numbers, l = math content, @{} removes left padding
1 & $\displaystyle gridDim.x = TC, \ 0 \leq blockIdx.x < TC$ \\[2pt] % extra space after row
2 & $\displaystyle blockDim.x = 256, \ 0 \leq threadIdx.x < 256$
\end{tabular}
\end{tcolorbox}
    \vspace{-0.1in}
    \subcaption{XXXX}
    \label{fig:running-b}
    
\end{minipage}%
\hfill
\begin{minipage}[t]{0.97\columnwidth}
\begin{tcolorbox}[colback=white!95!gray,% background color
boxrule=0.3pt, % thin border
left=0.5mm, right=0.5mm, top=0mm, bottom=0.2mm,
fontupper=\ttfamily\footnotesize,
valign=top, 
]
\noindent
\begin{tabular}{@{}r@{\quad }l} % r = line numbers, l = math content
1 & $\displaystyle threadIdx.x \leq \texttt{loop\_index0} < 896,$ \\
  & $\displaystyle (\texttt{loop\_index0} - threadIdx.x) \% 256 == 0$ \\[2pt]
2 & $\displaystyle blockIdx.x \times 896 < INT\_MAX$ \\[2pt]
3 & $\displaystyle 0 \leq \texttt{id} \times 16 < N_{i} \times S_{i} - 16$ \\[2pt]
4 & $\displaystyle (\texttt{loop\_index1} - threadIdx.x1) / 256$ \\
  & $\displaystyle== (\texttt{loop\_index0} - threadIdx.x) / 256$ \\[2pt]
5 & $\displaystyle threadIdx.x1 \neq threadIdx.x \lor blockIdx.x1 \neq blockIdx.x$ \\[2pt]
6 & $\displaystyle B_{r} + (blockIdx.x1 \times 896 + \texttt{loop\_index1}) \times 16$ \\
  & $\displaystyle \quad == B_{r} + (blockIdx.x \times 896 + \texttt{loop\_index0}) \times 16$ \\[2pt]
7 & $\displaystyle \texttt{loop\_index0\_out} \geq 896$
\end{tabular}
\end{tcolorbox}
    \vspace{-0.1in}
    \subcaption{XXXX}
    \label{fig:running-c}
\end{minipage}
    \mycaption{fig:running}{XXXXX.}
    {}
\end{figure}
